SCAN List Decoding of Polar Codes

In this paper we propose an enhanced soft cancellation (SCAN) decoder for polar codes based on decoding stages permutation. The proposed soft cancellation list (SCANL) decoder runs $L$ independent SCAN decoders, each one relying on a different permuted factor graph. The estimated bits are selected among the $L$ candidates through a dedicated metric provided by the decoders. Furthermore, we introduce an early-termination scheme reducing decoding latency without affecting error correction performance. We investigate the error-correction performance of the proposed scheme under various combinations of number of iterations used, permutation set and early-termination condition. Simulation results show that the proposed SCANL provides similar results when compared with belief propagation list, while having a smaller complexity. Moreover, for large list sizes, SCANL outperforms non-CRC aided successive cancellation list decoding.

==> figures/graph.tex <==

\begin{figure}[!t]
  \centering
\resizebox{0.47\textwidth}{!}{ \begin{tikzpicture}
[stack/.style={rectangle split, rectangle split parts=4, draw, anchor=center},
  myarrow/.style={single arrow, draw=none}]
  [->,>=stealth',shorten >=1pt,auto,
                    semithick]
\node[red,thick,inner sep=0pt,scale=0.8] (MBS){\MBS{MBS}} (0,2);
\node[stack,left= 2.2cm of MBS] (db) {$F_1$\nodepart{two}$F_2$\nodepart{three}$\cdots$\nodepart{four}$F_N$} (0,0);
\node[above= 0.1cm of db] {File Library};
\path (db.east) edge[thick,line width=0.7mm] node[above] {Core Network} (MBS.west);
%\node[circle,fill=red] at (2,2) {};
\node[scale=0.6]  at (-3,-3) (SBS1) {\BS{SBS$_1$}};
\node[scale=0.6]  at (-1,-3) (SBS2) {\BS{SBS$_2$}};
\node[scale=0.6]  at (1,-3) (SBS3) {\BS{SBS$_3$}};
\node[scale=0.6]  at (3,-3) (SBS4) {\BS{SBS$_4$}};
\node[stack,left= 0.1cm of SBS1,scale=0.6] (db1) {$1$\nodepart{two}$2$\nodepart{three}$\cdots$\nodepart{four}$M$};
\node[stack,left= 0.1cm of SBS2,scale=0.6] (db2) {$1$\nodepart{two}$2$\nodepart{three}$\cdots$\nodepart{four}$M$};
\node[stack,right= 0.1cm of SBS3,scale=0.6] (db3) {$1$\nodepart{two}$2$\nodepart{three}$\cdots$\nodepart{four}$M$};
\node[stack,right= 0.1cm of SBS4,scale=0.6] (db4) {$1$\nodepart{two}$2$\nodepart{three}$\cdots$\nodepart{four}$M$};
\node[fill=yellow!20,draw=none,text=red,circle]  at (-4,-6) (u1) {u$_1$};
\node[fill=yellow!20,draw=none,text=orange,circle]  at (-3,-6) (u2) {u$_2$};
\node[fill=yellow!20,draw=none,text=blue,circle]  at (-2,-6) (u3) {u$_3$};
\node[fill=yellow!20,draw=none,text=orange,circle]  at (-1,-6) (u4) {u$_4$};
\node [fill=yellow!20,draw=none,text=orange,circle]  at (0,-6) (u5) {u$_5$};
\node[fill=yellow!20,draw=none,text=green,circle]  at (1,-6) (u6) {u$_6$};
\node[fill=yellow!20,draw=none,text=green,circle]  at (2,-6) (u7) {u$_7$};
\node[fill=yellow!20,draw=none,text=green,circle]  at (3,-6) (u8) {u$_8$};
\node[fill=yellow!20,draw=none,text=green,circle]  at (4,-6) (u9) {u$_9$};
\path (SBS1.north) edge[thick,line width=0.5mm] node[left=1cm] {$\cdots$} (MBS.south);
\path (SBS2.north) edge[thick,line width=0.5mm] node {} (MBS.south);
\path (SBS3.north) edge[thick,line width=0.5mm] node {} (MBS.south);
\path (SBS4.north) edge[thick,line width=0.5mm] node[right=1cm] {$\cdots$} (MBS.south);
\path (SBS1) edge[->,red] node[left=0.2cm,text=black] {$\cdots$} (u1);
\path (SBS1) edge[->,yellow!80] node {} (u2);
\path (SBS1) edge[->,yellow!80] node {} (u5);
\path (SBS1) edge[->,blue] node {} (u3);
\path (SBS2) edge[->,yellow!80] node {} (u2);
\path (SBS2) edge[->,blue] node {} (u3);
\path (SBS2) edge[->,yellow!80] node {} (u4);
\path (SBS2) edge[->,yellow!80] node {} (u5);
\path (SBS2) edge[->,green] node {} (u6);
\path (SBS3) edge[->,yellow!80] node {} (u2);
\path (SBS3) edge[->,yellow!80] node {} (u4);
\path (SBS3) edge[->,blue] node {} (u3);
\path (SBS3) edge[->,green] node {} (u7);
\path (SBS3) edge[->,green] node {} (u8);
\path (SBS3) edge[->,green] node {} (u9);
\path (SBS4) edge[->,blue] node {} (u3);
\path (SBS4) edge[->,yellow!80] node {} (u4);
\path (SBS4) edge[->,yellow!80] node {} (u5);
\path (SBS4) edge[->,green] node {} (u6);
\path (SBS4) edge[->,green] node {} (u7);
\path (SBS4) edge[->,green] node {} (u8);
\path (SBS4) edge[->,green] node[right=0.2cm,text=black] {$\cdots$} (u9);
\end{tikzpicture}}
 \caption{Instantaneous Heterogeneous network topology.}
  \label{fig:graph}
\end{figure}

==> figures/square.tex <==
\def\firstcircle{(1,1) circle (1.7cm)}
\def\secondcircle{(1,-1) circle (1.7cm)}
\def\thirdcircle{(-1,-1) circle (1.7cm)}
\def\fourthcircle{(-1,1) circle (1.7cm)}
\def\rectangle{(-1,1) rectangle (1,-1)}
\begin{figure}[ht!]
  \centering
  \begin{tikzpicture}[scale=2]
  \clip (-1.5,-1.5) rectangle (1.5,1.5);
   \draw[black,fill=blue!20] (-1,1)
        rectangle (1,-1);

    \draw[fill=none,dashed,green] \firstcircle ;
    \draw[fill=none,dashed,green] \secondcircle;
    \draw[fill=none,dashed,green] \thirdcircle ;
 \draw[fill=none,dashed,green] \fourthcircle ;

    \begin{scope}
      \clip \rectangle;
      \fill[red!10] \firstcircle;
    \end{scope}
     \begin{scope}
      \clip \rectangle;
      \fill[red!10] \secondcircle;
    \end{scope}
     \begin{scope}
      \clip \rectangle;
      \fill[red!10] \thirdcircle;
    \end{scope}
    \begin{scope}
      \clip \rectangle;
      \fill[red!10] \fourthcircle;
    \end{scope}

    \begin{scope}
      \clip \rectangle;
      \clip \firstcircle;
      \fill[green!10] \secondcircle;
    \end{scope}

 \begin{scope}
      \clip \rectangle;
      \clip \firstcircle;
      \fill[green!10] \fourthcircle;
    \end{scope}
    
     \begin{scope}
      \clip \rectangle;
      \clip \thirdcircle;
      \fill[green!10] \secondcircle;
    \end{scope}
    
     \begin{scope}
      \clip \rectangle;
      \clip \thirdcircle;
      \fill[green!10] \fourthcircle;
    \end{scope}
    
     \begin{scope}
      \clip \rectangle;
      \clip \secondcircle;
      \clip \thirdcircle;
      \fill[yellow!10] \fourthcircle;
    \end{scope}
    
      \begin{scope}
      \clip \rectangle;
      \clip \secondcircle;
      \clip \thirdcircle;
      \fill[yellow!10] \firstcircle;
    \end{scope}
    
      \begin{scope}
      \clip \rectangle;
      \clip \firstcircle;
      \clip \fourthcircle;
      \fill[yellow!10] \secondcircle;
    \end{scope}
    
        \begin{scope}
      \clip \rectangle;
      \clip \firstcircle;
      \clip \fourthcircle;
      \fill[yellow!10] \thirdcircle;
    \end{scope}
    
          \begin{scope}
      \clip \rectangle;
      \clip \firstcircle;
      \clip \secondcircle;
      \clip \fourthcircle;
      \fill[blue!10] \thirdcircle;
    \end{scope}

\foreach \x in {1,...,3}{
\foreach \y in {1,...,3}{
\pgfmathparse{rand} \pgfmathsetmacro\xa{\pgfmathresult}
\pgfmathparse{rand}\pgfmathsetmacro\ya{\pgfmathresult} 
\draw [thick,fill=yellow!30] (\xa,\ya) circle (0.05cm);
}}
 
   \node[scale=0.9] at (-1,-1) {\BS{SBS$_1$}} {};
       % \draw[fill=none,dashed,green] (-1,-1) circle (1.7cm);
        \node[scale=0.9] at (-1,1) {\BS{SBS$_2$}} {};
      %  \draw[fill=none,dashed,green] (-1,1) circle (1.7cm);
        \node[scale=0.9] at (1,-1) {\BS{SBS$_3$}} {};
      %  \draw[fill=none,dashed,green] (1,-1) circle (1.7cm);
        \node[scale=0.9] at (1,1) {\BS{SBS$_4$}} {};
       % \draw[fill=none,dashed,green] (1,1) circle (1.7cm);
         \draw[fill=none,dashed,green] \firstcircle ;
    \draw[fill=none,dashed,green] \secondcircle;
    \draw[fill=none,dashed,green] \thirdcircle ;
 \draw[fill=none,dashed,green] \fourthcircle ;
   \end{tikzpicture}
  \caption{Small cells topology.}
  \label{fig:square}
\end{figure}


